Robotic Detection and Estimation of Single Scuba Diver Respiration Rate from Underwater Video

Human respiration rate (HRR) is an important physiological metric for diagnosing a variety of health conditions from stress levels to heart conditions. Estimation of HRR is well-studied in controlled terrestrial environments, yet robotic estimation of HRR as an indicator of diver stress in underwater for underwater human robot interaction (UHRI) scenarios is to our knowledge unexplored. We introduce a novel system for robotic estimation of HRR from underwater visual data by utilizing bubbles from exhalation cycles in scuba diving to time respiration rate. We introduce a fuzzy labeling system that utilizes audio information to label a diverse dataset of diver breathing data on which we compare four different methods for characterizing the presence of bubbles in images. Ultimately we show that our method is effective at estimating HRR by comparing the respiration rate output with human analysts.

==> TextFiles/acknowledgment.tex <==
\section*{Acknowledgment}
This work is indebted to the entire Interactive Robotics \& Vision Laboratory (IRVLab), specifically, Chelsey Edge, and Cory Ohnsted for assisting in data collection that made diver breathing possible, and Michael Fulton for his initial conception of the diver breathing project. Also, a special thanks must be given to Junaed Sattar for his conscientious guidance and support throughout the development of the diver respiration rate prediction system.

==> TextFiles/conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}

==> TextFiles/introduction.tex <==
\section{Introduction}
\label{sec:intro}
Human respiration rate (HRR) is an important physiological metric that is
ubiquitous in the medical community. It indicates a number of different
health phenomena such as human stress levels \cite{grossman1983respiration, giannakakis2019review}, exposure to external stimuli like extreme heat or cold \cite{tipton1999immersion}, lung-related health issues \cite{cretikos2008respiratory}, and heart conditions \cite{roppolo2009dispatcher, suess1980effects}. Measurement of HRR in controlled terrestrial environments is commonplace. Physicians often rely on plethysmography bands for accurate HRR assessments \cite{bricout2019adaptive}. These bands are wrapped around a patient's abdomen and utilize the expansion and contraction of the human torso to stress piezoelectric circuits that produce voltages which are correlated with respiration rate \cite{golpe2002home}. While these bands are excellent in controlled hospital settings, where the patient is often immobilized or confined to a bed, they do not work well in field environments. Other wearable technologies that show promise in field environments, such as optical wrist heart rate monitors \cite{aliverti2017wearable} or piezo-resistive fabric sensors \cite{jeong2009wearable} can be used to passively measure time differences between heart beats, which can then be correlated with HRR \cite{schafer2008estimation}. However, these contact-based wearables are unreliable underwater due to the movement and signal attenuation caused
by the layer of water between the optical signal and the user's skin. Exposure protection worn by scuba divers for underwater operations, such as drysuits and wetsuits, also prevents direct contact with the user's skin. Real time communication over Bluetooth or Wi-Fi is infeasible due to severe attenuation of these signals underwater.
HRR in the underwater environment for real-time health monitoring is therefore an open problem that is not easily accomplished using existing commercial technologies. \change Yet, the prevalence of underwater operations for diverse tasks like submerged pipeline inspections \cite{agbakwuru2012oil}, nuclear waste pool maintenance \cite{stark2023}, ship hull maintenance \cite{maclin1983overview}, and overhead environment rescues \cite{van2020deep} place humans under extreme environmental conditions that could lead to catastrophic injury or death. We thus argue that assessment of diver health by companion autonomous underwater vehicles (AUVs) is of paramount importance. \stopchange
% \vspace{-2mm} % arXiv version
\begin{figure}
    \centering
    \includegraphics[width=1.0\columnwidth]{figures/front_page_diver_breathing.png}
    \caption{Robotic estimation of diver respiration rate during a closed-water evaluation of the proposed detection system. The Aqua autonomous underwater vehicle \cite{dudek2007aqua} is using visual image data from a monocular camera and a ROS \cite{ROS2009ICRA} node implementation of the system in this paper to estimate the diver's respiration rate, shown in green text in the grayscale inset image.}
    \label{fig:example_graphic}
    \vspace{-5mm}
\end{figure}
% \vspace{-2mm}
These risks to humans are partially offset by advancements in AUV design, control \cite{lapierre2007nonlinear, yuh2000design}, perception \cite{islam2020fast}, communication \cite{cong2021underwater}, and navigation capabilities \cite{paull2013auv}. It is conceivable that in the near future AUVs will be used to support complex underwater human-robot interaction (UHRI) and teaming scenarios, where AUVs and humans equipped with scuba diving equipment will work together to accomplish physically and mentally challenging tasks \cite{bingham2010robotic, petillot2002real, modasshir2018coral, li2016vision}.  While significant research effort has been dedicated to improving robotic perception for scene understanding \cite{islam2019understanding}, context-aware diver approach strategies \cite{fulton2022using}, and communication technologies \cite{chiarella2015gesture}, to our knowledge, robotic visual detection of diver respiration rate is an unexplored area of research. 

There are two primary reasons we argue robotic detection of HRR is an important part of supporting complex UHRI scenarios. First, robots could use the information for situational awareness. A robot that can accurately detect HRR could, in theory, alert the diver when the diver is entering a distressed state or at risk for excess gas consumption that could lead to an out of air emergency \cite{anegg2002stress,lippmann2020scuba}. Second, a previous UHRI study \cite{fulton2023} indicates that exhalation of bubbles through a scuba diving regulator significantly diminshes the efficacy of visual and acoustic communication between robots and divers. Yet these are the primary mechanisms that show promise for UHRI communication strategies \cite{chavez2021underwater,fulton2019robot,fulton2022robot,enan2022}.


To accomplish detection and estimation of HRR, we argue that utilizing visual image data is an effective means for assessing underwater HRR by identifying images with bubbles. Bubbles are a positive indication that a diver is in an exhalation state. The temporal separation of exhalation states is an approximation of the duration of a single respiration cycle. By keeping track of respiration cycles, we can estimate the respiration rate. See Fig.~\ref{fig:example_graphic} for the respiration system described in this work running using the camera data extracted from the Aqua AUV.
% $DEBUG$ JOURNAL ARTICLE SENTENCE
% To minimize the potential for miscommunication from robot-to-human (R2H), robotic detection of HRR allows the robot to near-optimally time communication between exhalation cycles of the diver. Essentially, the robot waits until the diver is done exhaling and then proceeds to communicate the intended information.

Our primary contribution is the robotic visual estimation of HRR using a systematic approach that utilizes the timing of exhalation and inhalation cycles to estimate the respiration rate. We present results from training a custom support vector machine (SVM), convolutional neural network (CNN), and convolutional long short-term memory network (CNN-LSTM) using labeled diver breathing data created by a fuzzy labeling system. We also present results of estimated HRR in comparison to evaluations by humans. \change We show that given a fuzzy labeling strategy using audio-produced labels and conventional detection methods, we can predict respiration rate reasonably well so that it agrees with a human analyst's estimate.\stopchange

%% THE INFORMATION BELOW COULD BE USEFUL FOR A JOURNAL ARTICLE EXTENSION OF THIS WORK
% Yet, the underwater environment is precisely where monitoring a critical health indicator like HRR would be beneficial for safe operations. The underwater robotics community has long propounded the concept of the underwater robotic assistant (UWRA). These are robots that work alongisde human divers and in theory can provide arbitrarily complex support, spanning from delivering tools to divers to completing complex tasks on their own. While a tremendous amount of research has been dedicated to UWRA control mechanisms, hydrodynamics, localization, and path planning, a comparatively smaller effort has been dedicated to the support portion, which entails human-to-robot (H2R) and robot-to-human (R2H) communication methodologies. These are important because they represent at a very fundamental level the actual utility of a UWRA to human. A successful UHRI scenario is one in which R2H or H2R communication is enabled and realized without error in the communicated information. Many technologies have been propounded for enabling bi-directional communication, which include optical LED lights, hand signals or robotic movement that mimics human gestures, and acoustics. 

% All of the communication methodologies attempt to subvert some form of environmental challenge. For example, hand signals are used because they are common to diving operations and complex information can be encoded with relatively simple gestures; LED lights attempt to cut through dark or silted environments, where gestures are not visible; and finally acoustics work over long distances or instances in which neither LED lights nor gesture-based technologies would function. However, all of these technologies, especially acoustics, become exceedingly challenging for the human diver to perceive the communicated information when the diver is exhaling. 

% The process of exhalation from a scuba diving regulator creates noise that degrades both acoustically communicated information and visually communicated information. We subvert these challenges by accurately timing the communicated information based on the HRR cycles of inhalation and exhalation. We do this in two parts: 
% \begin{enumerate}
%     \item We extract the human respiration rate from video data and approximate the respiration cycle.
%     \item We perform a priority-based scheduling routine that utilizes the respiration cycle as a constraint input.
% \end{enumerate}

% Overall we show that accurately through our application, we can detect diver respiration rate, and we can utilize our predictions to optimally schedule information based on priority of the information.

==> TextFiles/problem_description.tex <==
\section{Problem Description}
\label{sec:problem_descr}
